A Formal Study on Backward Compatible Dynamic Software Updates

We study the dynamic software update problem for programs interacting with an environment that is not necessarily updated. We argue that such updates should be backward compatible. We propose a general definition of backward compatibility and cases of backward compatible program update. Based on our detailed study of real world program evolution, we propose classes of backward compatible update for interactive programs, which are included at an average of 32% of all studied program changes. The definitions of update classes are parameterized by our novel framework of program equivalence, which generalizes existing results on program equivalence to non-terminating executions. Our study of backward compatible updates is based on a typed extension of W language.

==> dsu-backward-compatibility.tex <==
\section{Backward compatibility}\label{sec:backwardComptibility}

\input{highlevel-prog-env-exec-spec}


\subsection{Hybrid executions and state mapping}

DSU is a process of updating software while it is running. This results in a hybrid execution in which part of the execution is that of the old program and part of the execution is for the new program. %~\cite{iuliandissertation, upstare_dissertation_09}.
%, aiming to reduce the cost of updating
%In general, updates may or may not include the environment (including users).

%\subsection{Hybrid executions and state mapping}

%%state mapping function: set of config. of old program P to set of config. of new program P'
%% the external state is copied without change
State mapping is a function $\delta$ mapping an internal state and a non-halt step of one program $P$ to an internal state and a step of another program $P'$, $\delta: \mathcal{M}_{int}^P \times (\mathcal{S}^P \setminus \{halt\}) \mapsto \mathcal{M}_{int}^{P'} \times \mathcal{S}^{P'}$.
%%
The external state is not mapped because the environment is not necessarily updated. In addition, we cannot change input and output that
already occurred and that I/O must be part of the hybrid execution.


%%DSU hybrid execution rely on state mapping
\begin{definition}\label{def:hybridExec} {\bf (Hybrid execution)}
A hybrid execution $(M_{{ext}_0}, I, \allowbreak C_P;C_{P'})$, produced by DSU using state mapping $\delta$ from program $P$
%$P = (\mathcal{S}^P, \mathcal{M}^P, M_{{int}_0}^P, s_0^P,\allowbreak \mathcal{I}, \mathcal{O})$
 to program $P'$,
 %$P'=(\mathcal{S}^{P'}, \mathcal{M}^{P'}, M_{{int}_0}^{P'}, s_0^{P'},\allowbreak \mathcal{I}', \mathcal{O}')$,
is an execution $(M_{{ext}_0}, I, C_P)$ of $P$ concatenated with an execution $(M_{ext}', I_r', C_{P'})$ of $P'$
where the first configuration $c_{P'} = ((M_{int}', M_{ext}'), s', i', I_r', IO')$ in $C_{P'}$ is obtained by applying the state mapping to the last configuration $c_{P} = ((M_{int}, M_{ext}), s(\neq halt), i, I_r, IO)$ in $C_{P}$ as follows:
\begin{itemize}
\item $(M_{int}', s') = \delta(M_{int}, s)$;

\item $(i' = i) \wedge (I_r' = I_r) \wedge (IO' = IO) \wedge (M_{ext} \subseteq M_{ext}')$.
\end{itemize}
\end{definition}
%% P and P' cannot be arbitrary different
%% I/O of P is subset of P', every in M_ext is a part of some external state of P'
%Because it is impossible to change known or occurred I/O, inputs and occurred I/O are copied to the configuration of $P'$; every external state of $P$ has to be a part of some external state of $P'$ because the environment may not be updated; we have no restriction as to the initial internal state and initial step between $P$ and $P'$.


%%%correctness of hybrid execution
\subsection{Backward compatibility}

In this paper, we consider updates in which the environment is not necessarily updated.
%Also, we are modeling updating a program with well established user base to its following release,
%in which changes between two programs are not arbitrary.
%% state mapping
%DSU results in {\em hybrid executions} where part of the execution is of an old program and part of the execution is of the updated program by mapping the configuration of the old program to a configuration of the new program; this is the state mapping problem.
%%backward compatiblity
It follows that in order for the hybrid execution to be meaningful, the new program should provide functionality expected by both old and new users of the system. %%
%In this section, we formally define hybrid execution with state mapping in DSU and the backward compatibility.
%Since DSU mechanism is not of interest in this paper, we skip the formal definition of DSU.


%%IO sequence correctness
In practice, specifications are not explicitly available. Instead, the program is its own specification. This means that the specification that the program satisfies can only be inferred by the external behavior of the program.
Bug fixes create a dilemma for dynamic software updates. When a program has a bug, its external behavior does not captures its
 {\em implicit specification} and the update will change the behavior of the program. In what follows, we first discuss what flexibility we can be afforded for a backward compatible update and then we give formal definitions of backward compatibility and state our assumptions for allowing bug fixes.

%We use the external behavior of a statically updated program as the reference specification against which the dynamic update is to be judged.
%% clear execution: either totally old or totally new
%For executions terminated before DSU, these executions should satisfy the specification of old programs;
%for executions started after DSU, these executions should satisfy the specification of new program.
%% hybrid
%As to hybrid executions going through DSU, these execution should satisfy the implicit specification of the old program because users interacting with hybrid executions are not necessarily updated; this is backward compatibility in this paper.

%%factors affecting correctness of hybrid execution.
We consider a hybrid execution starting from a program
$P = (\mathcal{S}, \mathcal{M}_{int} \times \mathcal{M}_{ext}, M_{{int}_0}, s_0, \mathcal{I}, \mathcal{O})$
and being updated to a program
$P' = (\mathcal{S}', \mathcal{M}_{int}' \times \mathcal{M}_{ext}', M_{{int}_0}', s_0', \mathcal{I}', \mathcal{O}')$.
We examine how the two programs should be related for a meaningful hybrid execution.
\begin{enumerate}
\item (Inputs)
Input set $\mathcal{I}'$ of $P'$ should be a superset of that $\mathcal{I}$ of $P$ to allow for {\em old users} to interact with $P'$
	after the update.
It is possible to allow for new input values in $\mathcal{I}'$ to accommodate new functionality under the assumption
	that old users do not generate new input values. Such new input values should be expected to produce erroneous output by old users
	as they are not part of $P$'s specification.

\item (Outputs)
Output produced by $P'$ should be identical to output produced by $P$ if all the input in an execution comes from the input set of $P$.
This is needed to ensure that interactions between old users and the program $P'$ can make sense from the perspective of old users.
This is true in the case that the update does not involve a bug fix, but what should be done if the update indeed involves a bug fix and
	the output produced by the old program was not correct to start with?
As far as syntax, a bug fix should not introduce new output values. As far as semantics, we should allow the bug fix to change what
	output is produced for a given input. We discuss this further under the bug fix heading.
In summary, if we ignore bug fixes, the new program should behave as the old program when provided with input meant for the old program.
	
	%Output values $\mathcal{O}'$ of $P'$ are a super set of $\mathcal{O}$ of $P$ because users interact with the hybrid execution is not necessarily updated.
    %  Though the specification of program $P$ is defined based on output values $\mathcal{O}$ of $P$, we assume that hybrid executions produce output values in $\mathcal{O}'$.
  %    Unlike inputs, we allow new outputs produced by $P'$ in case some bugfix results in these new outputs.
 %     We do not explicitly mention what new outputs are allowed in hybrid executions because it is in general related to a set of I/O history inherently expressed in program's steps. We speculate bugfix from the difference between $\mathcal{S}$ and $\mathcal{S}'$. Bugfix is correcting the specification of program $P$ in its rare executions. In this sense, the hybrid execution is not violating the old specification based on I/O of $P$ by allowing new outputs from bugfix in $P'$.

%	because users interact with the hybrid execution is not necessarily updated and the possible new functionality.
    %% remaining inputs: no new inputs
   % Because (a) new functionality is independent of existing functionality and (b) bugfix does not introduce new inputs, we assume that the remaining inputs are all in $\mathcal{I}$. So is the input in the state of last configuration of $P$ in the hybrid execution.
    %% discuss if allowing new inputs or interpret old input in different way
    % We do not allow users to give new inputs in $P'$, $\mathcal{I}'\setminus\mathcal{I}$, which in general introduce new behavior not mentioned in specification of $P$.
    %% new meaning of old inputs values? how to express that?
   % When only receiving inputs in $\mathcal{I}$ of $P$, we assume that $P'$ and $P$ produce the same I/O sequence if $P'$ only introduce new functionalities based on $P$.

\item (Bugfix)
Handling bug fixes is problematic. If the produced output already violates the fix, then there is no way for the hybrid execution
	to satisfy the {\em implicit semantics} of the program or the semantics of the new program.
Some bug fixes can be handled. For example, a bug that causes a program to crash for some input can be fixed to allow the program
	to continue executing. Applying the fix to a program that has not encountered the bug should not be problematic.
Another case is when the program should terminate for some input sequence, but the old program does not terminate.
A bug fix that allows the program to terminate should not present a semantic difficulty for old users.

In general, we assume that there are  {\em valid} executions and {\em invalid} executions of the old program.
I/O sequences produced in {invalid} executions are not in specification of the program.
We assume that an invalid execution will lead to an {\em error} configuration not explicitly handled by the program developers.
%Error configurations are those where the state are of unexpected values with respect to the next step to execute.
%% need to explain static update earlier
We do not expect the state mapping to change an error configuration into an non-error configuration just as static updating does not fix occurred errors. Besides, we do not attempt to determine if a particular configuration is an error configuration.
Such determination is not possible in general and very hard in practice.
We simply assume that the configuration at the time of the update is not an error configuration.
(which is equivalent to assuming the existence of an oracle $\mathcal{J}_P$ to determine if  a particular configuration is erroneous,
$\mathcal{J}_P(C_P)$ = true if the configuration $C_P$ is not erroneous).
%We do not be aware of other obvious better strategy for handling error configuration.

\item (New functionality) New functionality is usually accompanied by new inputs/outputs and the expansion of external state. We assume that new functionality is independent of existing functionality in the sense that programs $P$ and $P'$ produce the same I/O sequence when receiving inputs in $\mathcal{I}$ only.
    We therefore assume all new inputs $\mathcal{I}'\setminus\mathcal{I}$ are introduced by new functionality.
    %based on the above discussion of bugfix.

Every external state of $P$ is part of some external state of program $P'$ because of the definition of the specification of $P$. We only consider expansion of the external state of $P$ for new functionalities in $P'$ where the expansion of external state is independent of values in existing external state. One of the motivating examples is to add application settings for new program feature.
\end{enumerate}


In light of the discussion above we give the following definition of backward compatibility in the absence of bug fixes.

%With respect to the discussion of factors with impact on correctness of hybrid execution and under the assumption of users not necessarily updated, we differentiate backward compatibility depending on if there is bugfix between the old program and the updated program.
\begin{definition}\label{def:bwdcomptGeneral} {\bf (Backward compatible hybrid executions)}
Let $P = (\mathcal{S}, \mathcal{M}_{int} \times \mathcal{M}_{ext}, M_{{int}_0}, s_0, \mathcal{I}, \mathcal{O})$ be a program satisfying a specification $\Sigma$.
We say that a hybrid execution $(M_{ext}, I, C_P;C_P')$ from $P$ to a program
$P' = (\mathcal{S}', \mathcal{M}_{int}' \times \mathcal{M}_{ext}', M_{{int}_0}', s_0', \mathcal{I}', \mathcal{O}')$ is backward compatible with implicit specification of $P$ if all of the following hold:
\begin{itemize}
\item The last configuration in $C_P$ is not an error configuration, $C_P = ``C';(M, s', i, I_r, IO)" : \mathcal{J}_P(C_P)$=true.

\item The hybrid execution satisfies the specification $\Sigma$ of $P$,

\noindent$\Sigma(M_{ext}, I, IO(C_P;C_P')) = true$;

\item Inputs/outputs/external states of $P$ are a subset of those of $P': \mathcal{I} \subseteq \mathcal{I}', \mathcal{O} \subseteq \mathcal{O}' \text{ and } \mathcal{M}_{ext} \subseteq \mathcal{M}_{ext}'$;
\end{itemize}
\end{definition}

If there is bug fix between programs $P'$ and $P$, we need to adapt Definition~\ref{def:bwdcomptGeneral} to allow for
some executions on input sequences from $\mathcal{I}$ to violate the specification of $P$. Above we identified two cases in
which bug fixes are safe (replacing a response with no response or replacing a no response with a correct response without
introducing new output values). We omit the definition.

%The hybrid execution satisfies
 %\begin{enumerate}
 %\item either
 %the specification $\Sigma$ of $P: \Sigma(M_{ext}, IO(C_P;C_P')) = true$;

 %\item or
 %the fixed specification $\Sigma'$ but not $\Sigma$, $\Sigma': \mathcal{M}_{ext} \times seq(\mathcal{I}\cup\mathcal{O}') \mapsto \{true, false\}$ ,
 %$(\Sigma'(M_{ext}, IO(C_P;C_P')) = true) \wedge (\Sigma(M_{ext}, IO(C_P;C_P')) = false)$;
 %\end{enumerate}

%The only difference between $\Sigma'$ and $\Sigma$ is the difference of outputs admitted by implicit specification of $P$ due to bugfix in program $P'$.

%% hybrid execution with bugfix covers the definition of hybrid exec. with bugfix-free
%The definition of backward compatible hybrid execution with bugfix fully covers that of backward compatible bugfix-free hybrid execution. In the following, any mention of backward compatible hybrid execution refers to the definition for hybrid executions with bugfix.

%%backward compatible updates
We have the backward compatible updates by extending the definition of a backward compatible hybrid execution to all possible hybrid executions.
\begin{definition}\label{def:bcupdates} {\bf (Backward compatible updates)}
We say an updated program $P'$ is backward compatible with a program $P$ in configuration $C$ if there is hybrid execution, from configuration $C$ of $P$ to $P'$ that is backward compatible with specification of $P$.
\end{definition}


\subsection{Backward compatible program behavior changes}
With the formal definition of backward compatibility,
it is desirable to check what behavior changes of an updated program help ensure a safe update.
%Based on our programming language, the interaction between a program and its environment is represented by I/O sequence which is essentially the observational behavior of the program.
Backward compatibility is essentially a relation between I/O sequences produced by an old program and those produced by an updated program. We summarized typical possibilities of the relation into six cases in Figure~\ref{NewProgBehaviorFig} by considering consequence of major update motivation (i.e., new functionality, bug fix and program perfective/preventive needs~\cite{iso14764}).
According to David Parnas~\cite{Parnas94}, a program is updated to adapt to changing needs.
In other words, program changes are to produce more or less or different output according to changing needs. These changes are captured by case 2, 3, 4, 5 and 6 in Figure~\ref{NewProgBehaviorFig}.
We also capture output-preserving changes which are most likely motivated by the program developer's own needs (e.g., software maintainability),
which is case 1 in Figure~\ref{NewProgBehaviorFig}.
%Case 7 in Figure~\ref{NewProgBehaviorFig} is for all other new program behavior.

%We decompose the adaptation changes into new functionality and/or bug fix.

%\begin{figure}
%		\begin{center}
%			\begin{tabular}{| c | l |}
%                \hline
%				Case          & New program behavior                                         \\ \hline
%				1             & the old behavior                                             \\ \hline
%				2             & the old behavior for old input and consuming inputs          \\
%                              & that are only from new clients                               \\ \hline
%                3             & producing more output while the old program terminates       \\ \hline
%				4             & termination while the old program produces erroneous output  \\ \hline
%				5             & eliminating unwanted arbitrary behavior                      \\ \hline
%				6             & different output that is functionally equivalent to old output     \\ \hline
%%				7             & all other different behavior that is unknown why it is different from old behavior                                             \\ \hline
%			\end{tabular}
%		\end{center}
%		\caption{Six cases of general new program behavior}\label{NewProgBehaviorFig}
%\end{figure}

\begin{figure}
		\begin{center}
			\begin{tabular}{| c | l |}
                \hline
				Case          & Formal new program behavior                                         \\ \hline
                 1            & the old behavior including external state extension: \\
				              & $\Sigma_{P} \subseteq \Sigma_{P'}$,
                                 or $\Sigma_{P'}$ = \{$(M_{ext'}, \text{oneseq}(\mathcal{I}), \text{oneseq}(\mathcal{I}\cup\mathcal{O})) \rightarrow \text{val}$       \\
                              & $| \exists (M_{ext}, \text{oneseq}(\mathcal{I}), \text{oneseq}(\mathcal{I}\cup\mathcal{O})) \rightarrow \text{val}$
                                 in $\Sigma_{P}$ \\
                              &  and $M_{ext} \subseteq M_{ext'}$ \} where $\mathcal{I} = \mathcal{I'}$, $\mathcal{O} = \mathcal{O'}$
                                  and $\mathcal{M}_{ext} \subseteq \mathcal{M}_{ext'}$    \\ \hline

                 2            & the old behavior for old input and consuming inputs \\
                              & that are only from new clients:                               \\
				              & $\Sigma_{P} \subseteq \Sigma_{P'} \land$ \\
                              &   $\Sigma_{P'} \setminus \Sigma_{P}$ =
                                     \{$({M}_{ext}, \text{oneseq}(\mathcal{I'}), \text{oneseq}(\mathcal{I'} \cup \mathcal{O'})) \rightarrow \text{true}$ \\
                              &   $| \, \text{oneseq}(\mathcal{I'} \cup \mathcal{O'}) \text{ includes at least one input in } (\mathcal{I}' \setminus \mathcal{I})$\} $\neq \emptyset$ \\
                              & where $\mathcal{I} \subset \mathcal{I'}$, $\mathcal{O} \subseteq \mathcal{O'}$
                                  and $\mathcal{M}_{ext} = \mathcal{M}_{ext'}$    \\ \hline

                 3            & producing more output while the old program terminates:      \\
                              & $\Sigma_{P'} \setminus \Sigma_{P}$ =
                                   $\{(M_{ext}, \text{oneseq}(\mathcal{I}), \text{oneseq}(\mathcal{I}\cup\mathcal{O})) \mapsto \text{false}$  \\
                              & $| (M_{ext}, \text{oneseq}(\mathcal{I}), \text{oneseq}(\mathcal{I}\cup\mathcal{O})) \in \Delta_{f} \neq \emptyset\}$ \\
                              & $\cup$ $\{(M_{ext}, \text{oneseq}(\mathcal{I}), \text{oneseq}(\mathcal{I}\cup\mathcal{O})\centerdot\text{oneseq'}(\mathcal{I}\cup\mathcal{O})) \mapsto \text{true}$ \\
                              & $| (M_{ext}, \text{oneseq}(\mathcal{I}), \text{oneseq}(\mathcal{I}\cup\mathcal{O})\centerdot\text{oneseq'}(\mathcal{I}\cup\mathcal{O})) \in \Delta_{t} \neq \emptyset\}$ \\
                              & $\Sigma_{P} \setminus \Sigma_{P'}$ =
                                   $\{(M_{ext}, \text{oneseq}(\mathcal{I}), \text{oneseq}(\mathcal{I}\cup\mathcal{O})) \mapsto \text{false}$  \\
                              & $| (M_{ext}, \text{oneseq}(\mathcal{I}), \text{oneseq}(\mathcal{I}\cup\mathcal{O})) \in \Delta_{t} \neq \emptyset\}$ \\
                              & $\cup$ $\{(M_{ext}, \text{oneseq}(\mathcal{I}), \text{oneseq}(\mathcal{I}\cup\mathcal{O})\centerdot\text{oneseq'}(\mathcal{I}\cup\mathcal{O})) \mapsto \text{true}$ \\
                              & $| (M_{ext}, \text{oneseq}(\mathcal{I}), \text{oneseq}(\mathcal{I}\cup\mathcal{O})\centerdot\text{oneseq'}(\mathcal{I}\cup\mathcal{O})) \in \Delta_{f} \neq \emptyset\}$ \\
                              & where $\mathcal{I} = \mathcal{I'}$, $\mathcal{O} = \mathcal{O'}$
                                  and $\mathcal{M}_{ext} = \mathcal{M}_{ext'}$    \\ \hline

                 4            & termination while the old program produces erroneous output: \\
				              & $\Sigma_{P'} \setminus \Sigma_{P}$ =
                                   $\{(M_{ext}, \text{oneseq}(\mathcal{I}), \text{oneseq}(\mathcal{I}\cup\mathcal{O})) \mapsto \text{true}$  \\
                              & $| (M_{ext}, \text{oneseq}(\mathcal{I}), \text{oneseq}(\mathcal{I}\cup\mathcal{O})) \in \Delta_{t} \neq \emptyset\}$ \\
                              & $\cup$ $\{(M_{ext}, \text{oneseq}(\mathcal{I}), \text{oneseq}(\mathcal{I}\cup\mathcal{O})\centerdot\text{oneseq'}(\mathcal{I}\cup\mathcal{O})) \mapsto \text{false}$ \\
                              & $| (M_{ext}, \text{oneseq}(\mathcal{I}), \text{oneseq}(\mathcal{I}\cup\mathcal{O})\centerdot\text{oneseq'}(\mathcal{I}\cup\mathcal{O})) \in \Delta_{f} \neq \emptyset\}$ \\

                              & $\Sigma_{P} \setminus \Sigma_{P'}$ =
                                   $\{(M_{ext}, \text{oneseq}(\mathcal{I}), \text{oneseq}(\mathcal{I}\cup\mathcal{O})) \mapsto \text{true}$  \\
                              & $| (M_{ext}, \text{oneseq}(\mathcal{I}), \text{oneseq}(\mathcal{I}\cup\mathcal{O})) \in \Delta_{f} \neq \emptyset\}$ \\
                              & $\cup$ $\{(M_{ext}, \text{oneseq}(\mathcal{I}), \text{oneseq}(\mathcal{I}\cup\mathcal{O})\centerdot\text{oneseq'}(\mathcal{I}\cup\mathcal{O})) \mapsto \text{false}$ \\
                              & $| (M_{ext}, \text{oneseq}(\mathcal{I}), \text{oneseq}(\mathcal{I}\cup\mathcal{O})\centerdot\text{oneseq'}(\mathcal{I}\cup\mathcal{O})) \in \Delta_{t} \neq \emptyset\}$ \\
                              & where $\mathcal{I} = \mathcal{I'}$, $\mathcal{O} = \mathcal{O'}$
                                  and $\mathcal{M}_{ext} = \mathcal{M}_{ext'}$    \\ \hline

                5             & eliminating unintentional arbitrary behavior:    \\
				              & $\Sigma_{P'} \setminus \Sigma_{P}$ =
                                   $\{(M_{ext}, \text{oneseq}(\mathcal{I}), \text{oneseq}(\mathcal{I}\cup\mathcal{O})) \mapsto \text{false}$  \\
                              & $| (M_{ext}, \text{oneseq}(\mathcal{I}), \text{oneseq}(\mathcal{I}\cup\mathcal{O})) \in \Delta_{arbi} \neq \emptyset\}$ \\
                              & $\Sigma_{P} \setminus \Sigma_{P'}$ =
                                   $\{(M_{ext}, \text{oneseq}(\mathcal{I}), \text{oneseq}(\mathcal{I}\cup\mathcal{O})) \mapsto \text{true}$  \\
                              & $| (M_{ext}, \text{oneseq}(\mathcal{I}), \text{oneseq}(\mathcal{I}\cup\mathcal{O})) \in \Delta_{arbi} \neq \emptyset\}$ \\
                              & where $\mathcal{I} = \mathcal{I'}$, $\mathcal{O} = \mathcal{O'}$
                                  and $\mathcal{M}_{ext} = \mathcal{M}_{ext'}$    \\ \hline

                6             & different output that is functionally equivalent to old output: \\
				              & $(\Sigma_{P} \neq \Sigma_{P'}) \land (\Sigma_{P} \equiv \Sigma_{P'})$     \\
                              &   where $\mathcal{I} = \mathcal{I'}$,
                                        $(\mathcal{O} \neq \mathcal{O'}) \land (\mathcal{O} \equiv \mathcal{O'})$
                                  and $\mathcal{M}_{ext} = \mathcal{M}_{ext'}$    \\ \hline
			\end{tabular}
		\end{center}
		\caption{Six cases of formalized general new program behavior}\label{NewProgBehaviorFig}
\end{figure}


%\begin{figure}
%		\begin{center}
%			\begin{tabular}{| c | l |}
%                \hline
%				Update motivation class            & Resulting new program behavior class        \\ \hline
%				new functionality                  & 1, 2, 3                                     \\ \hline
%                bug fix                           & 1, 3, 4, 5                                  \\ \hline
%                performance optimization          & 1, 6                                        \\ \hline
%			\end{tabular}
%		\end{center}
%		\caption{New program behavior classes for major update motivation classes}\label{NewProgBehaviorForMajorMotivationFig}
%\end{figure}

Furthermore, we find that an update is {\em backward compatible} if in every execution the new program behavior is one of the six cases in Figure~\ref{NewProgBehaviorFig}.
Cases 1 and 2 are obviously backward compatible because an old client is guaranteed to get old responses.
Cases 3, 4, 5, and 6 are not obviously backward compatible.
In general, we consider backward compatibility under general assumption of program semantics as opposed to specific assumptions of semantics.
Case 3 is backward compatible because we assume the change is either adding new functionality, or fixing a bug in which the old program hanged or crashed. Similarly, case 4 is backward compatible.
In case 5 the program changes usually imply bug fix.
Then case 5 is backward compatible because the new program keeps correct old behavior.
Case 6 is backward compatible because different I/O interaction could express the same application semantics. For example, a greeting message could be changed from ``hi" to ``hello".

%why only these 6 types: the possible change of I/O sequence between the new and the old
Except the six cases of backward compatibility, other new program behavior is not recognized to be backward compatible because it is unclear what causes the difference and how the different new behavior corresponds to old behavior in general.
The motivation for unrecognized new behavior could be unidentified bug fixes
that are application dependent.
%There are no more cases because the eight cases are all the possibilities of a relation between two program-produced I/O sequences.
Furthermore, bug fixes modify the behavior of a program and, in the absence of information to the contrary, one cannot in general distinguish them  from other functionality changes.
In conclusion, it is not possible to go much beyond the six backward compatibility cases.

%%valid init state
%In general, every program has a set of valid initial states for all possibly valid executions of the program. In a broad sense, valid initial states are included in the states of no error. We therefore do not make the distinction of valid initial states explicitly.

%%summary
%Backward compatibility is a property of two programs and the hybrid execution from one program to the other regarding the consistent external behavior for users that are not necessarily updated.


==> equiv-term-behavior-supporting-lemmas-LoopLessLikelyToTerm.tex <==
%%#######################################less likely to termination##################################################
%loop less likely to terminate

%the lemma says about the specific form of configuration that occurs
\begin{lemma}\label{lmm:ExistenceOfIthIterStart}
One while statement $s = ``\text{while}_{\langle n\rangle}(e) \{S\}"$ starts in a state $m(\mathfrak{f}, m_c)$ in which the loop counter of $s$ is zero, $m_c(n) = 0$ and the crash flag is not set, $\mathfrak{f} = 0$. For any positive integer $i$, if there is a state $m'(m_c')$ reachable from $m$ in which the loop counter is $i$, $m_c'(n) = i$, then there is a configuration $(S;s, m''(\mathfrak{f}'', m_c''))$ reachable from the configuration $(s, m)$ in which loop counter of $s$ is $i$, $m_c''(n) = i$ and the crash flag is not set, $\mathfrak{f}'' = 0$:

$\forall i>0\,:\, ({((s, m(\mathfrak{f}, m_c)) ->* (S', m'(\mathfrak{f'}, m_c')))} \, \wedge \,
                    (m_c(n) = 0) \, \wedge \,
                    (\mathfrak{f} = 0) \, \wedge \,
                    (m_c'(n) = i)) => $

$(s, m(\mathfrak{f}, m_c)) ->* (S;s, m''(\mathfrak{f}, m_c''))$ where $\mathfrak{f} = 0$ and $m_c''(n) = i$.
\end{lemma}
\begin{proof}
The proof is by induction on $i$.

{\bf Base case} $i=1$.

We show that the evaluation of the loop predicate of $s$ w.r.t the value store $\vals$ in the state $m(m_c, \vals)$ produces an nonzero integer value. By our semantic rule, if the evaluation of the predicate expression of $s$ raises an exception, the execution of $s$ proceeds as follows:

\begin{tabbing}
xxxxx\=xxxx\=\kill
\>\>     $({s}, m(\mathfrak{f}, m_c,\vals))$\\
\>= \>   $(\text{while}_{\langle n\rangle} (e) \; \{S\}, {m(m_c, \vals)})$\\
\>$->$\> $(\text{while}_{\langle n\rangle} (\text{error}) \; \{S\}, {m(m_c, \vals)})$ by the EEval rule\\
\>$->$\> $(\text{while}_{\langle n\rangle} (0) \; \{S\}, {m(1/\mathfrak{f}, m_c, \vals)})$ by the ECrash rule\\
\>{\kStepArrow [k] }\> $(\text{while}_{\langle n\rangle} (0) \; \{S\}, m(1/\mathfrak{f}, m_c))$ for any $k>0$, by the Crash rule.
\end{tabbing}

Hence, we have a contradiction that there is no configuration in which the loop counter of $s$ is 1.


When the evaluation of the loop predicate expression of $s$ produce zero, the execution of $s$ proceeds as follows:

\begin{tabbing}
xxxxx\=xxxx\=\kill
\>\>     $({s}, m(\mathfrak{f}, m_c,\vals))$\\
\>= \>   $(\text{while}_{\langle n\rangle} (e) \; \{S\}, {m(m_c, \vals)})$\\
\>$->$\> $(\text{while}_{\langle n\rangle} (0) \; \{S\}, {m(m_c, \vals)})$ by the EEval rule\\
\>$->$\> $({\text{skip}}, m(m_c[0/n_1]))$ by the Wh-F rule.
\end{tabbing}

Hence, we have a contradiction that there is no configuration in which the loop counter of $s$ is 1.
The evaluation of the predicate expression of $s$ w.r.t value store $\vals$ produce nonzero value.
The execution of $s$ proceeds as follows:

\begin{tabbing}
xxxxx\=xxxx\=\kill
\>\>     $({s}, m(\mathfrak{f}, m_c,\vals))$\\
\>= \>   $(\text{while}_{\langle n\rangle} (e) \; \{S\}, {m(\mathfrak{f}, m_c, \vals)})$\\
\>$->$\> $(\text{while}_{\langle n\rangle} (\mathcal{E}\llbracket e\rrbracket\vals) \; \{S\}, {m(\mathfrak{f}, m_c, \vals)})$ by the EEval rule\\
\>$->$\> $({S;\text{while}_{\langle n\rangle} (e) \; \{S\}}, m(\mathfrak{f}, m_c[1/n_1], \vals))$ by the Wh-T rule.
\end{tabbing}

The lemma holds.

{\bf Induction step}.

The hypothesis IH is that, if there is a configuration $(S', m_i(m_c^i))$ reachable from $(s, m)$ in which the loop counter of $s$ is $i$, $m_c^i(n) = i>0$, then there is a reachable configuration $(S;s, m_i(\mathfrak{f}, m_c^i))$ from $(s, m)$ where the loop counter of $s$ is $i$ and the crash flag is not set.

Then we show that, if there is a configuration $(S', m_{i+1}(m_c^{i+1}))$ reachable from $(s, m)$ in which the loop counter of $s$ is $i+1$, then there is a reachable configuration $(S;s, m_{i+1}(\mathfrak{f}, m_c^{i+1}))$ from $(s, m)$ where the loop counter of $s$ is $i+1$ and the crash flag $\mathfrak{f}$ is not set.

By Lemma~\ref{lmm:loopCntStepwiseInc}, the loop counter of $s$ is increasing by one in one step. Hence, there must be one configuration reachable from $(s, m)$ in which the loop counter of $s$ is $i$.
By hypothesis, there is the configuration $(S;s, m_{i}(\mathfrak{f}, m_c^i, \vals_i))$ reachable from $(s, m)$ in which the loop counter is $i$, $m_c^i(n) = i$, and the crash flag is not set, $\mathfrak{f} = 0$.
By the assumption of unique loop labels, $s\notin S$. Then the loop counter of $s$ is not redefined in the execution of $S$ started in state $m_{i}(\mathfrak{f}, m_c^i, \vals_i)$. Because there is a configuration in which the loop counter of  $s$ is $i+1$, then the execution of $S$ when started in the state $m_{i}(\mathfrak{f}, m_c^i, \vals_i)$ terminates,
$(S, m_{i}(\mathfrak{f}, m_c^i, \vals_i)) ->* (\text{skip}, m_{i+1}(\mathfrak{f}, m_c^{i+1}, \vals_{i+1}))$ where
$\mathfrak{f} = 0$ and $m_c^{i+1}(n) = i$.
By Corollary~\ref{coro:termSeq},
$(S;s, m_{i}(\mathfrak{f}, m_c^i, \vals_i)) ->* (s, m_{i+1}(\mathfrak{f}, m_c^{i+1}, \vals_{i+1}))$.
By similar argument in base case, the evaluation of the predicate expression w.r.t the value store $\vals_{i+1}$ produce nonzero integer value. The execution of $s$ proceeds as follows:

\begin{tabbing}
xxxxx\=xxxx\=\kill
\>\>     $(s, m_{i+1}(\mathfrak{f}, m_c^{i+1}, \vals_{i+1}))$\\
\>= \>   $(\text{while}_{\langle n\rangle} (e) \; \{S\}, {m_{i+1}(\mathfrak{f}, m_c^{i+1}, \vals_{i+1})})$\\
\>$->$\> $(\text{while}_{\langle n\rangle} (\mathcal{E}\llbracket e\rrbracket\vals_{i+1}) \; \{S\}, {m_{i+1}(\mathfrak{f}, m_c^{i+1}, \vals_{i+1})})$ by the EEval rule\\
\>$->$\> $({S;\text{while}_{\langle n\rangle} (e) \; \{S\}}, {{m_{i+1}(\mathfrak{f}, m_c^{i+1}[(i+1)/n], \vals_{i+1})}})$ by the Wh-T rule.
\end{tabbing}
The lemma holds.
\end{proof}

%the main intermediate lemma for less likely to terminate for two loop stmt
\begin{lemma}\label{lmm:loopLessLikelyTermCondIntermediate}
Let $s_1 = ``\text{while}_{\langle n_1\rangle}(e) \{S_1\}"$ and
    $s_2 = ``\text{while}_{\langle n_2\rangle}(e) \{S_2\}"$ be two while statements and all of the following hold:
\begin{itemize}
\item The termination deciding variables of $s_2$ are a subset of those of $s_1$,
$\text{TVar}(s_2) \subseteq \text{TVar}(s_1)$.

\item The loop body $S_1$ of $s_1$ and $S_2$ of $s_2$ satisfy the syntactic condition of equivalent computation of variables in $\text{TVar}(s_2)$,
 $\forall x \in \text{TVar}(s_2)\,:\, S_1 \equiv_{x}^s S_2$.

\item The loop body $S_1$ of $s_1$ is less likely to terminate than $S_2$ of $s_2$ when started in states in which crash flags are not set and whose value stores agree on the values of variables in $\text{TVar}(S_2)$,
$\forall m_{S_1}(\mathfrak{f}_{1}, \vals_{S_1})\, m_{S_2}(\mathfrak{f}_{2}, \vals_{S_2}):$

$((\forall x \in \text{TVar}(S_2), \vals_{S_1}(x) = \vals_{S_2}(x)) \wedge
 (\mathfrak{f}_1 = \mathfrak{f}_2 = 0)) =>
 ((S_1, m_{S_1}(\mathfrak{f}_1, \vals_{S_1})) \leq_{H} (S_2, m_{S_2}(\mathfrak{f}_2, \vals_{S_2})))$.
\end{itemize}

If $s_1$ and $s_2$ start in states
$\state_1(\mathfrak{f}_1, m_c^1, \vals_1)$ and $\state_2(\mathfrak{f}_2, m_c^2, \vals_2)$ respectively, and
crash flags are not set, $\mathfrak{f}_1 = \mathfrak{f}_2 = 0$,
$s_1$ and $s_2$ have not started in states $m_1$ and $m_2$ (initial loop counter is zero), $m_c^1(n_1) = m_c^2(n_2) = 0$
and the value stores $\vals_1$ and $\vals_2$ agree on the values of the termination deciding variables of $s_2$, $\forall x \in \text{TVar}(s_2)\,:\, \vals_1(x) = \vals_2(x)$,
then, for any positive integer $i$,
if there is a configuration $(s_1, m_{1_i}(\mathfrak{f}_1, m_c^{1_i}, \vals_{1_i}))$ reachable from $(s_1, m_1)$
such that crash flags are not set, the loop counters of $s_1$ is $i$, then
there is a configuration $(s_2, m_{2_i}(\mathfrak{f}_2, m_c^{2_i}, \vals_{2_i}))$ reachable from $(s_2, m_2)$ in which
crash flag is not set, the loop counter of $s_2$ is $i$ and value stores $\vals_{1_i}$ and $\vals_{2_i}$ agree on the values of variables in $\text{TVar}(s_2)$:

%$\forall m_1 \, m_2\,:\,$

\noindent$({(s_1, m_1(\mathfrak{f}_1, m_c^1, \vals_1)) ->* (s_1, m_{1_i}(\mathfrak{f}_1, m_c^{1_i}, \vals_{1_i}))} \wedge
 (m_c^1(n_1) = m_c^2(n_2) = 0) \wedge
 (\forall x \in \text{TVar}(s_2), \vals_1(x) = \vals_2(x)) \wedge
 (\mathfrak{f}_1 = \mathfrak{f}_2 = 0) \wedge
 (m_c^{1_i}(n_1) = i)) =>$
$(s_2, m_2(\mathfrak{f}_2, m_c^2, \vals_2)) ->* (s_2, m_{2_i}(\mathfrak{f}_2, m_c^{2_i}, \vals_{2_i}))$ where
\begin{itemize}
\item $\mathfrak{f}_2 = 0$; and


\item $m_c^{2_i}(n_2) = i$; and


\item $\forall x \in \text{TVar}(s_2)\,:\, \vals_{2_i}(x) = \vals_{1_i}(x)$.
\end{itemize}
\end{lemma}
\begin{proof}
%\noindent{\bf Proof}
By induction on $i$ .

\noindent{\bf Base case} $i = 1$.

We show that evaluations of the predicate expression of $s_1$ and $s_2$ produce same value w.r.t. value stores $\vals_1$ and $\vals_2$.
By the definition of loop variables, variables used in the predicate expression of $s_2$ are a subset of variables in the loop variables of $s_2$, $\text{Use}(e) \subseteq \text{LVar}(s_2)$.
By assumption, $\forall x \in \text{Use}(e), \vals_1(x) = \vals_2(x)$.
By the property of expression meaning function $\mathcal{E}$, $\mathcal{E}\llbracket e\rrbracket\vals_1 = \mathcal{E}\llbracket e\rrbracket\vals_2$. By assumption, there is configuration that the loop counter of $s_1$ is 1.
Then,  $\mathcal{E}\llbracket e\rrbracket\vals_1 = \mathcal{E}\llbracket e\rrbracket\vals_2 \notin \{\text{error}, 0\}$.
The execution of $s_1$ proceeds as follows.

\begin{tabbing}
xxxxx\=xxxx\=\kill
\>\>     $({s_1}, m_{1}(m_c^1, \vals_1))$\\
\>= \>   $(\text{while}_{\langle n_1\rangle} (e) \; \{S_1\}, {m_{1}(m_c^{1}, \vals_1)})$\\
\>$->$\> $(\text{while}_{\langle n_1\rangle} (\mathcal{E}\llbracket e\rrbracket\vals_1) \; \{S_1\}, {m_{1}(m_c^{1}, \vals_1)})$
by the EEval rule\\
\>$->$\> $({S_1;\text{while}_{\langle n_1\rangle} (e) \; \{S_1\}}, m_1(m_c^{1}[1/n_1], \vals_1))$ by the Wh-T rule.
\end{tabbing}

Similar, the execution of $s_2$ proceeds to
$({S_2;\text{while}_{\langle n_1\rangle} (e) \; \{S_2\}}, m_2(m_c^{2}[1/n_2], \vals_2))$.

By assumption, there is configuration $(s_1, m_{1_1}(\mathfrak{f}_1, m_c^{1_1}, \vals_{1_1}))$ where $m_c^{1_1}(n_1) = 1$.
Hence, the execution of $S_1$ when started in state $m_1(m_c^{1}[1/n_1], \vals_1)$ terminates,
$(S_1, m_1(m_c^{1}[1/n_1], \vals_1)) ->* (\text{skip}, m_{1'}(\mathfrak{f}_1, m_c^{1'}, \vals_{1'}))$.

We show that state $m_{1'}(\mathfrak{f}_1, m_c^{1'}, \vals_{1'})$ is the same as
$m_{1_1}(\mathfrak{f}_1, m_c^{1_1}, \vals_{1_1})$ by contradiction.
We assume that $m_{1'}(\mathfrak{f}_1, m_c^{1'}, \vals_{1'}) \neq m_{1_1}(\mathfrak{f}_1, m_c^{1_1}, \vals_{1_1})$.

By Corollary~\ref{coro:termSeq},
$({S_1;\text{while}_{\langle n_1\rangle} (e) \; \{S_1\}}, m_1(m_c^{1}[1/n_1], \vals_1)) ->*
 (\text{while}_{\langle n_1\rangle} (e) \; \{S_1\}, m_{1'}(\mathfrak{f}_1, m_c^{1'}, \vals_{1'}))$

\noindent $ = (s_1, m_{1'}(\mathfrak{f}_1, m_c^{1'}, \vals_{1'}))$.
Then, the configuration
$(s_1, m_{1_1}(\mathfrak{f}_1, m_c^{1_1}, \vals_{1_1}))$ must be reachable from

\noindent$(s_1, m_{1'}(\mathfrak{f}_1, m_c^{1'}, \vals_{1'}))$.
By the assumption of unique loop labels, $S_1\notin s_1$. By Corollary~\ref{lmm:loopCntRemainsSame},
$m_c^{1'}(n_1) = m_c^{1}(n_1) = 1$.
By semantic rules, there are three possibilities regarding the evaluations of the predicate expression of $s_1$.
\begin{enumerate}
%eval crash
\item $\mathcal{E}\llbracket e\rrbracket\vals_{1'} = \text{error}$.

The execution of $s_1$ proceeds as follows:

\begin{tabbing}
xxxxx\=xxxx\=\kill
\>\>     $({s_1}, {m_{1'}(\mathfrak{f}_1, m_c^{1'}, \vals_{1'})})$\\
\>= \>   $(\text{while}_{\langle n_1\rangle} (e) \; \{S_1\}, {m_{1'}(\mathfrak{f}_1, m_c^{1'}, \vals_{1'})})$\\
\>$->$\> $(\text{while}_{\langle n_1\rangle} (\text{error}) \; \{S_1\}, {m_{1'}(\mathfrak{f}_1, m_c^{1'}, \vals_{1'})})$
by the EEval rule\\
\>$->$\> $({\text{while}_{\langle n_1\rangle} (0) \; \{S_1\}}, {m_{1'}(1/\mathfrak{f}_1, m_c^{1'}, \vals_{1'})})$ by the ECrash rule\\
\>{\kStepArrow [i] }\> $({S_1;\text{while}_{\langle n_1\rangle} (0) \; \{S_1\}}, {m_{1'}(1/\mathfrak{f}_1, m_c^{1'}, \vals_{1'})})$ for any $i>0$, by the Crash rule.
\end{tabbing}

We have a contradiction that there is no configuration $(s_1, m_{1_1}(\mathfrak{f}_1, m_c^{1_1}, \vals_{1_1}))$ where
$\mathfrak{f}_1 = 0 \wedge m_c^{1_1}(n_1) =1$.

%eval zero
\item $\mathcal{E}\llbracket e\rrbracket\vals_{1'} = 0$.

The execution of $s_1$ proceeds as follows:
\begin{tabbing}
xxxxx\=xxxx\=\kill
\>\>     $({s_1}, {m_{1'}(\mathfrak{f}_1, m_c^{1'}, \vals_{1'})})$\\
\>= \>   $(\text{while}_{\langle n_1\rangle} (e) \; \{S_1\}, {m_{1'}(\mathfrak{f}_1, m_c^{1'}, \vals_{1'})})$\\
\>$->$\> $(\text{while}_{\langle n_1\rangle} (0) \; \{S_1\}, {m_{1'}(\mathfrak{f}_1, m_c^{1'}, \vals_{1'})})$
by the EEval rule\\
\>$->$\> $({\text{skip}}, {m_{1'}(m_c^{1'}[0/n_1], \vals_{1'})})$ by the Wh-F rule.
\end{tabbing}

We have a contradiction that there is no configuration $(s_1, m_{1_1}(\mathfrak{f}_1, m_c^{1_1}, \vals_{1_1}))$ where
$\mathfrak{f}_1 = 0 \wedge m_c^{1_1}(n_1) =1$.

%eval nonzero, no crash
\item $\mathcal{E}\llbracket e\rrbracket\vals_{1'} \notin \{0, \text{error}\}$.

The execution of $s_1$ proceeds as follows:

\begin{tabbing}
xxxxx\=xxxx\=\kill
\>\>     $({s_1}, {m_{1'}(\mathfrak{f}_1, m_c^{1'}, \vals_{1'})})$\\
\>= \>   $(\text{while}_{\langle n_1\rangle} (e) \; \{S_1\}, {m_{1'}(\mathfrak{f}_1, m_c^{1'}, \vals_{1'})})$\\
\>$->$\> $(\text{while}_{\langle n_1\rangle} (\mathcal{E}\llbracket e\rrbracket\vals_{1'}) \; \{S_1\}, {m_{1'}(\mathfrak{f}_1, m_c^{1'}, \vals_{1'})})$ by the EEval rule\\
\>$->$\> $({S_1;\text{while}_{\langle n_1\rangle} (e) \; \{S_1\}}, {m_{1'}(m_c^{1'}[2/n_1], \vals_{1'})})$ by the Wh-T rule.
\end{tabbing}

We have a contradiction that there is no configuration $(s_1, m_{1_1}(\mathfrak{f}_1, m_c^{1_1}, \vals_{1_1}))$ where
$\mathfrak{f}_1 = 0 \wedge m_c^{1_1}(n_1) =1$.
\end{enumerate}

In summary, the state ${m_{1'}(\mathfrak{f}_1, m_c^{1'}, \vals_{1'})} = {m_{1_1}(\mathfrak{f}_1, m_c^{1_1}, \vals_{1_1})}$.

By assumption, value stores $\vals_1$ and $\vals_2$ agree on values of variables in $\text{TVar}(s_2)$:
$\forall x \in \text{TVar}(s_2)\,:\, \vals_1(x) = \vals_2(x)$.
$S_1$ terminates when started in the state $m_1(m_c^{1}[1/n_1], \vals_1)$.
Hence, by assumption, $S_2$ terminates when started in the state $m_2(m_c^{2}[1/n_2], \vals_2)$:
$(S_2, m_2(m_c^{2}[1/n_2], \vals_2)) ->* (\text{skip}, m_{2'}(m_c^{2'}, \vals_{2'}))$.
%%
By the assumption of unique loop labels, $s_2 \notin S_2$.
By Corollary~\ref{lmm:loopCntRemainsSame},
$m_c^{2'}(n_2) = m_c^{2}(n_2) = 1$.
%%
We show that value stores $\vals_{2'}$ and $\vals_{1_1}$ agree on values of variables in $\text{TVar}(s_2)$.
By Lemma~\ref{lmm:sameImpfromEquivCompCond}, $\text{Imp}(S_2, \text{TVar}(s_2)) = \text{Imp}(S_1, \text{TVar}(s_2))$.
We show that $\text{Imp}(S_2, \text{LVar}(s_2)) \subseteq \text{LVar}(s_2)$.

%\begin{tabbing}
%xxxxx\=xxxx\=\kill
%\>\>     $\text{LVar}(s_2)$\\
%\>=\>    $\text{Imp}(s_2,  \text{LVar}(S_2) \cup \text{Use}(e))$ by the definition of loop variables\\
%\>=\>    $\bigcup_{j\geq0} \text{Imp}(S_2^j, \text{LVar}(S_2) \cup \text{Use}(e))$  (1) by the definition of imported variables.\\
%\end{tabbing}

\begin{tabbing}
xxxxx\=xxxx\=\kill
\>\>              $\text{Imp}(S_2, \text{LVar}(s_2))$ \\
\>=\>             $\text{Imp}(S_2, \text{Imp}(s_2,  \text{LVar}(S_2) \cup \text{Use}(e)))$ by the definition of loop variables\\
\>=\>             $\text{Imp}(S_2, \bigcup_{j\geq0} \text{Imp}(S_2^j, \text{LVar}(S_2) \cup \text{Use}(e)))$ by the definition of imported variables\\
\>=\>             $\bigcup_{j\geq0}\text{Imp}(S_2, \text{Imp}(S_2^j, \text{LVar}(S_2) \cup \text{Use}(e)))$ by Lemma~\ref{lmm:impVarUnionLemma}\\
\>=\>             $\bigcup_{j>0}\text{Imp}(S_2^j, \text{LVar}(S_2) \cup \text{Use}(e))$ by Lemma~\ref{lmm:ImpPrefixLemma}\\
\>$\subseteq$\>   $\bigcup_{j\geq0} \text{Imp}(S_2^j, \text{LVar}(S_2) \cup \text{Use}(e))$ \\
\>=\>             $\text{Imp}(s_2, \text{LVar}(S_2) \cup \text{Use}(e)) = \text{LVar}(s_2)$.
\end{tabbing}

Similarly, we show that $\text{Imp}(S_2, \text{CVar}(s_2)) \subseteq \text{CVar}(s_2)$.
Hence, $\text{Imp}(S_2, \text{TVar}(s_2)) \subseteq \text{TVar}(s_2)$.
By Theorem~\ref{thm:equivCompMain}, value stores $\vals_{2'}$ and $\vals_{1_1}$ agree on values of variables in $\text{TVar}(s_2)$.




\noindent{\bf Induction step}.

\noindent The induction hypothesis IH is that, for $i (> 0)$,
if there is a configuration $(s_1, m_{1_i}(\mathfrak{f}_1, m_c^{1_i}, \vals_{1_i}))$ reachable from $(s_1, m_1)$
such that crash flag is not set, the loop counter of $s_1$ is $i$,
%%
then there is a configuration $(s_2, m_{2_i}(\mathfrak{f}_2, m_c^{2_i}, \vals_{2_i}))$ reachable from $(s_2, m_2)$ in which
crash flag is not set, the loop counter of $s_2$ is $i$ and value stores $\vals_{1_i}$ and $\vals_{2_i}$ agree on the values of variables in $\text{TVar}(s_2)$:

$({(s_1, m_1(\mathfrak{f}_1, m_c^1, \vals_1)) ->* (s_1, m_{1_i}(\mathfrak{f}_1, m_c^{1_i}, \vals_{1_i}))} \wedge
 (m_c^1(n_1) = m_c^2(n_2) = 0) \wedge
 (\forall x \in \text{TVar}(s_2), \vals_1(x) = \vals_2(x)) \wedge
 (\mathfrak{f}_1 = \mathfrak{f}_2 = 0) \wedge
 (m_c^{1_i}(n_1) = i)) =>$

$ (s_2, m_2(\mathfrak{f}_2, m_c^2, \vals_2)) ->* (s_2, m_{2_i}(\mathfrak{f}_2, m_c^{2_i}, \vals_{2_i}))$ where
\begin{itemize}
\item $\mathfrak{f}_2 = 0$; and


\item $m_c^{2_i}(n_2) = i$; and


\item $\forall x \in \text{TVar}(s_2)\,:\, \vals_{2_i}(x) = \vals_{1_i}(x)$.
\end{itemize}

Then we show that,
if there is a configuration $(s_1, m_{1_{i+1}}(\mathfrak{f}_1, m_c^{1_{i+1}}, \vals_{1_{i+1}}))$ reachable from $(s_1, m_1)$
such that the crash flag is not set, the loop counters of $s_1$ is $i+1$,
%%
then there is a configuration

\noindent$(s_2, m_{2_{i+1}}(\mathfrak{f}_2, m_c^{2_{i+1}}, \vals_{2_{i+1}}))$ reachable from $(s_2, m_2)$ in which
crash flag is not set, the loop counter of $s_2$ is $i+1$ and value stores $\vals_{1_{i+1}}$ and $\vals_{2_{i+1}}$ agree on the values of variables in $\text{TVar}(s_2)$:

$({(s_1, m_1(\mathfrak{f}_1, m_c^1, \vals_1)) ->* (s_1, m_{1_{i+1}}(\mathfrak{f}_1, m_c^{1_{i+1}}, \vals_{1_{i+1}}))} \wedge
 (m_c^1(n_1) = m_c^2(n_2) = 0) \wedge
 (\forall x \in \text{TVar}(s_2), \vals_1(x) = \vals_2(x)) \wedge
 (\mathfrak{f}_1 = \mathfrak{f}_2 = 0) \wedge
 (m_c^{1_{i+1}}(n_1) = i+1)) =>$

$ (s_2, m_2(\mathfrak{f}_2, m_c^2, \vals_2)) ->* (s_2, m_{2_{i+1}}(\mathfrak{f}_2, m_c^{2_{i+1}}, \vals_{2_{i+1}}))$ where
\begin{itemize}
\item $\mathfrak{f}_2 = 0$; and


\item $m_c^{2_{i+1}}(n_2) = i+1$; and


\item $\forall x \in \text{TVar}(s_2)\,:\, \vals_{2_{i+1}}(x) = \vals_{1_{i+1}}(x)$.
\end{itemize}

We show that there is a configuration $(s_1, m_{1_i}(\mathfrak{f}_{1}, m_c^{1_i}, \vals_{1_i}))$ reachable from $(s_1, m_1)$
such that the crash flag is not set, the loop counter of $s_1$ is $i$.
By Lemma~\ref{lmm:loopCntStepwiseInc}, every step of the execution of $s_1$ is increasing the loop counter of $s_1$ by one at most.
Therefore, there must exist one configuration reachable from $(s_1, m_1)$ in which the loop counter of $s_1$ is $i$ and the crash flag is not set. By Lemma~\ref{lmm:ExistenceOfIthIterStart}, there is a configuration $(S_1;s_1, m_i(\mathfrak{f}_1, m_c^i, \vals_i))$ reachable from the configuration $(s_1, m_1)$ in which the crash flag is not set, $\mathfrak{f}_1 = 0$, the loop counter of $s_1$ is $i$.

Because there is a configuration in which the loop counter of $s_1$ is $i+1$, then the execution of $S_1$ when started in the state
$m_{1_i}(\mathfrak{f}_1, m_c^{1_i}, \vals_{1_i})$ terminates,
$(S_1, m_{1_i}(\mathfrak{f}_{1}, m_c^{1_i}, \vals_{1_i})) ->* (\text{skip}, m_{1_{i'}}(\mathfrak{f}_{1}, m_c^{1_{i'}}, \vals_{1_{i'}}))$ where $\mathfrak{f}_{1} = 0$ and $m_c^{1_{i'}}(n_1) = i$.
This is because the loop counter of $s_1$ is not redefined in the execution of $S_1$ by Corollary~\ref{coro:loopCntRemainsSame} due to the fact that $s_1 \notin S_1$ by the assumption of unique loop labels.
By Corollary~\ref{coro:termSeq},
$(S_1;s_1, m_{1_i}(\mathfrak{f}_{1}, m_c^{1_i}, \vals_{1_i})) ->*
(s_1, m_{1_{i'}}(\mathfrak{f}_{1}, m_c^{1_{i'}}, \vals_{1_{i'}}))$ where
$\mathfrak{f}_{1} = 0$ and $m_c^{1_{i'}}(n_1) = i$.


By the induction hypothesis IH, there is a configuration $(s_2, m_{2_{i'}}(\mathfrak{f}_{2}, m_c^{2_{i'}}, \vals_{2_{i'}}))$
where
\begin{itemize}
\item $\mathfrak{f}_{1} = \mathfrak{f}_{2} = 0$; and


\item $m_c^{1_{i'}}(n_1) = m_c^{2_{i'}}(n_2) = i$; and


\item $\forall x \in \text{TVar}(s_2)\,:\, \vals_{1_{i'}}(x) = \vals_{2_{i'}}(x)$.
\end{itemize}

Then, by the similar argument in base case, we have that evaluations of the predicate expression of $s_1$ and $s_2$ w.r.t value stores $\vals_{1_{i'}}$ and $\vals_{2_{i'}}$ produce same nonzero value. Then the execution of $s_1$ proceeds as follows:

\begin{tabbing}
xxxxx\=xxxx\=\kill
\>\>                   $(s_1, m_{1_{i'}}(\mathfrak{f}_{1}, m_c^{1_{i'}}, \vals_{1_{i'}}))$\\
\>= \>                 $(\text{while}_{\langle n_1\rangle}(e) \; \{S_1\}, m_{1_{i'}}(\mathfrak{f}_{1}, m_c^{1_{i'}}, \vals_{1_{i'}}))$ \\
\>$->$\>               $(\text{while}_{\langle n_1\rangle}(v) \; \{S_1\}, m_{1_{i'}}(\mathfrak{f}_{1}, m_c^{1_{i'}}, \vals_{1_{i'}}))$ by the EEval rule \\
\>$->$\>               $(S_1;\text{while}_{\langle n_1\rangle}(e) \; \{S_1\}, m_{1_{i'}}(\mathfrak{f}_{1}, m_c^{1_{i'}}[(i+1)/n_1], \vals_{1_{i'}}))$ by the Wh-T rule.
\end{tabbing}

Similarly, execution of $s_2$ proceeds as follow:

\noindent$(s_2, m_{2_{i'}}(\mathfrak{f}_{2}, m_c^{2_{i'}}, \vals_{2_{i'}}))$ {\kStepArrow [2] }
$(S_2;s_2, m_{2_{i'}}(\mathfrak{f}_{2}, m_c^{2_{i'}}[(i+1)/n_2], \vals_{2_{i'}}))$.


By the similar argument in base case, we have the execution of $S_1$ when started in the state

\noindent$m_{1_{i'}}(\mathfrak{f}_{1}, m_c^{1_{i'}}[(i+1)/n_1], \vals_{1_{i'}})$ terminates,

\noindent$(S_1, m_{1_{i'}}(\mathfrak{f}_{1}, m_c^{1_{i'}}[(i+1)/n_1], \vals_{1_{i'}})) ->*
 (\text{skip}, m_{1_{i+1}}(\mathfrak{f}_{1}, m_c^{1_{i+1}}, \vals_{1_{i+1}}))$ where the loop counter of $s_1$ is $i+1$ and the crash flag is not set, $m_c^{1_{i+1}}(n_1) = i+1$.
It follows that, the execution of $S_2$ when started in the state
$m_{2_{i'}}(\mathfrak{f}_{2}, m_c^{2_{i'}}[(i+1)/n_2], \vals_{2_{i'}})$ terminates,

\noindent$(S_2, m_{2_{i'}}(\mathfrak{f}_{2}, m_c^{2_{i'}}[(i+1)/n_2], \vals_{2_{i'}})) ->*
 (\text{skip}, m_{2_{i+1}}(\mathfrak{f}_{2}, m_c^{2_{i+1}}, \vals_{2_{i+1}}))$ where:
\begin{itemize}
\item The crash flag is not set, $\mathfrak{f}_{2} = 0$; and

\item
 The loop counter of $s_2$ is $i+1$, $m_c^{2_{i+1}}(n_2) = i+1$; and

\item Value stores $\vals_{1_{i+1}}$ and $\vals_{2_{i+1}}$ agree on values of variables in $\text{TVar}(s_2)$:
$\forall x \in \text{TVar}(s_2)\,:\, \vals_{1_{i+1}}(x) = \vals_{2_{i+1}}(x)$.
\end{itemize}

 By Corollary~\ref{coro:termSeq},
 $(S_2;s_2, m_{2_{i'}}(\mathfrak{f}_{2}, m_c^{2_{i'}}[(i+1)/n_2], \vals_{2_{i'}})) ->*
 (s_2, m_{2_{i+1}}(\mathfrak{f}_{2}, m_c^{2_{i+1}}, \vals_{2_{i+1}}))$.

The lemma holds.
\end{proof}

\begin{lemma}\label{lmm:loopLessLikelyTermCond}
Let $s_1 = ``\text{while}_{\langle n_1\rangle}(e) \{S_1\}"$ and
    $s_2 = ``\text{while}_{\langle n_2\rangle}(e) \{S_2\}"$ be two while statements and all of the following hold:
\begin{itemize}
\item The termination deciding variables of $s_2$ are a subset of those of $s_1$,
$\text{TVar}(s_2) \subseteq \text{TVar}(s_1)$.

\item The loop body $S_1$ of $s_1$ and $S_2$ of $s_2$ satisfy the syntactic condition of equivalent computation of variables in $\text{TVar}(s_2)$,
 $\forall x \in \text{TVar}(s_2)\,:\, S_1 \equiv_{x}^s S_2$.

\item The loop body $S_1$ of $s_1$ is less likely to terminate than $S_2$ of $s_2$ when started in states in which crash flags are not set and whose value stores agree on the values of variables in $\text{TVar}(S_2)$,
$\forall m_{S_1}(\mathfrak{f}_{1}, \vals_{S_1})\, m_{S_2}(\mathfrak{f}_{2}, \vals_{S_2}):$

$((\forall x \in \text{TVar}(S_2), \vals_{S_1}(x) = \vals_{S_2}(x)) \wedge
 (\mathfrak{f}_1 = \mathfrak{f}_2 = 0)) =>
 ((S_1, m_{S_1}(\mathfrak{f}_1, \vals_{S_1})) \leq_{H} (S_2, m_{S_2}(\mathfrak{f}_2, \vals_{S_2})))$.
\end{itemize}

If $s_1$ and $s_2$ start in states
$\state_1(\mathfrak{f}_1, m_c^1, \vals_1)$ and $\state_2(\mathfrak{f}_2, m_c^2, \vals_2)$ respectively, such that
crash flags are not set, $\mathfrak{f}_1 = \mathfrak{f}_2 = 0$,
$s_1$ and $s_2$ have not started in states $m_1$ and $m_2$ (initial loop counter is zero), $m_c^1(n_1) = m_c^2(n_2) = 0$
and the value stores $\vals_1$ and $\vals_2$ agree on the values of variables in $s_2$, $\forall x \in \text{TVar}(s_2)\,:\, \vals_1(x) = \vals_2(x)$,
%%
if $s_1$ terminates when started in the state   $m_1(m_c^1, \vals_1)$,
then $s_2$ terminates when started in the state $m_2(m_c^2, \vals_2)$:
$\big((s_1, m_1(\mathfrak{f}_{1}, m_c^1, \vals_1)) ->* (\text{skip}, m_1'(\mathfrak{f}_{1}))\big) \wedge
      (\mathfrak{f}_{1} = \mathfrak{f}_{2} = 0) \wedge
      (\forall x \in \text{TVar}(s_2), \vals_1(x) = \vals_2(x)) \wedge
      (m_c^1(n_1) = m_c^2(n_2) = 0)
      =>
 \big((s_2, m_2(\mathfrak{f}_{2}, m_c^2, \vals_2)) ->* (\text{skip}, m_2'(\mathfrak{f}_{2}))\big)$ where $\mathfrak{f}_{2} = 0$.
\end{lemma}
\begin{proof}
By the definition of terminating execution, there are finite number of steps in the execution of $s_1$ when started in the state $m_1$. By Lemma~\ref{lmm:loopCntStepwiseInc}, there exists a finite positive integer $k$ such that the loop counter of $s_1$ is less than $k$. In the following, we consider $k$ to be the smallest positive integer such that the loop counter of $s_1$ is less than $k$. There are two possibilities:
\begin{enumerate}
\item $k = 1$.

Because $s_1$ terminates, then the evaluation of the predicate expression of $s_1$ w.r.t value store $\vals_1$ produce either zero or a nonzero integer value. Because $k$ is the smallest positive integer such that the loop counter of $s_1$ is less than $k$. Then the evaluation of the predicate expression of $s_1$ w.r.t value store $\vals_1$ produces zero.
In the proof of Lemma~\ref{lmm:loopLessLikelyTermCondIntermediate}, we show that evaluations of the predicate expression of $s_1$ and $s_2$ w.r.t value stores $\vals_1$ and $\vals_2$ produce same value. Hence, $s_2$ terminates.

\item  $k > 1$.

Because $k$ is the smallest positive integer such that the loop counter of $s_1$ is less than $k$. Then the loop counter of $s_1$ is less than or equal to $k-1$.
Then, by Lemma~\ref{lmm:ExistenceOfIthIterStart}, there exists a configuration $(S_1;s_1, m_{1_{k-1}}(\mathfrak{f}_{1}, m_c^{1_{k-1}}))$ reachable from the initial configuration $(s_1, m_1)$ in which the loop counter is $k-1$ and the crash flag is not set.

Because $s_1$ terminates when started in the state $m_1$, then $S_1$ terminates when started in the state $m_{1_{k-1}}(\mathfrak{f}_{1}, m_c^{1_{k-1}})$,
$(S_1, m_{1_{k-1}}(\mathfrak{f}_{1}, m_c^{1_{k-1}})) ->*
 (\text{skip}, m_{1_{k-1}'}(\mathfrak{f}_{1}, m_c^{1_{k-1}'}))$ where the crash flag is not set, $\mathfrak{f}_{1} = 0$.
 By the assumption of our unique labels, $s\notin S$, by Corollary~\ref{coro:loopCntRemainsSame}, loop counter of $s_1$ is not redefined in the execution of $S_1$ when started in the state $m_{1_{k-1}}(\mathfrak{f}_{1}, m_c^{1_{k-1}})$. Hence, the loop counter of $s_1$ is $k-1$ after the full execution of $S_1$, $m_c^{1_{k-1}'}(n_1) = k-1$.
 By Corollary~\ref{coro:termSeq},
 $(S_1;s_1, m_{1_{k-1}}(\mathfrak{f}_{1}, m_c^{1_{k-1}})) ->*
 (s_1, m_{1_{k-1}'}(\mathfrak{f}_{1}, m_c^{1_{k-1}'}, \vals_{1_{k-1}'}))$.
 By Lemma~\ref{lmm:loopLessLikelyTermCondIntermediate}, there is a configuration $(s_2, {m_{2_{k-1}'}(\mathfrak{f}_{2}, m_c^{2_{k-1}'}, \vals_{2_{k-1}'})})$ reachable from $(s_2, m_2)$ in which
 \begin{itemize}
 \item $\mathfrak{f}_{2} = 0$; and

 \item $m_c^{2_{k-1}'}(n_2) = k-1$; and

 \item $\forall x \in \text{TVar}(s_2)\,:\, \vals_{2_{k-1}'}(x) = \vals_{1_{k-1}'}(x)$.
 \end{itemize}

In the proof of Lemma~\ref{lmm:loopLessLikelyTermCondIntermediate},
 the evaluation of the predicate expression of $s_1$ and $s_2$ w.r.t value stores
 $\vals_{1_{k-1}'}$ and $\vals_{2_{k-1}'}$ produces same value. Because $s_1$ terminates and $k$ is the smallest positive integer such that the loop counter of $s_1$ is less than $k$. Then evaluations of of the predicate expression of $s_1$ and $s_2$ w.r.t value stores
 $\vals_{1_{k-1}'}$ and $\vals_{2_{k-1}'}$ produces zero. In conclusion, $s_2$ terminates.
\end{enumerate}
\end{proof} 

==> formal-back-comp-def.tex <==
\section{Formal Backward Compatibility}
Based on the general definition(Definition~\ref{def:bcupdates}) of backward compatibility and the concrete language model, we adapt the definition of backward compatibility by having a purely I/O specification.
%%informal description
Informally, we say a program $S_2$ to be backward compatible with a program $S_1$ if $S_2$ can produce the same {\em output sequence}, the same I/O sequence {till any corresponding output value}, produced in the program $S_1$'s valid executions.
We assume that all executions of $S_1$ are valid unless we can speculate bugfix from the difference between $S_2$ and $S_1$.
We care about the I/O sequence instead of the sequence of only outputs due to possible crashes from the lack of input.
%% the primitive for definition of backward compatibility
We use one primitive $``\text{Out}(\vals)"$ to represent the output sequence in value store $\vals$, the I/O sequence $\vals({id}_{IO})$ till the rightmost output value. When there is no output value in the I/O sequence $\vals({id}_{IO})$, $\text{Out}(\vals) = \varnothing$.
%% the formal definition
The definition of backward compatibility w.r.t our concrete language is as follows:
% same output sequence
\begin{definition}\label{def:backwardComptibilityConcrete} {\bf (Backward compatibility)}
We say that a statement sequence $S_2$ in a program $P_2$ when started in a state $m_2$ is backward compatible with $S_1$ in $P_1$ when started in a state $m_1$,
written $(S_1, m_1)  \subseteq_{O} (S_2, m_2)$, iff
$\forall m_1'$ such that there is valid execution
$(S_1, m_1) ->* ({S_1'}, m_1'(\vals_{1}'))$,
%%
there exists a state $m_2''$ reachable from the initial state $m_2$,
$({S_2}, m_2)\allowbreak ->* ({S_2''}, m_2''(\vals_{2}''))$ so that
$\text{Out}(\vals_{2}'') = \text{Out}(\vals_{1}')$.
\end{definition}

We present typical updates and show that updated programs with each of these updates are backward compatible with the old program.
We roughly divide updates into two categories based on if additional assumptions are required in the proof of backward compatibility (Definition~\ref{def:backwardComptibilityConcrete}).
\begin{enumerate}
\item The first category of updates include: variable renaming, statement reordering, statement duplication (e.g., loop distribution or loop fusion) and log-related change. As to logging, we use variables to model the log file in our concrete model. The proof of updates in the first category does not require additional assumptions.
    %%differentiate renaming with other updates
    As to variable renaming, two programs are alpha equivalent if there is only variable renaming between them. Then backward compatibility is implied trivially.
    %% definition of all updates together
    We do not formulate each of statement reordering, statement duplication and log-related change separately, we instead use a set of closely-knitted syntactic definitions for the three updates.
    %% showing equivalence
    Instead of showing backward compatibility directly, we show programs with updates in the first category are producing equivalent output sequence.

\item The second category of updates include updates that require different assumptions to establish the backward compatibility. Because we need distinct assumption for each update, we formulate each update and show the backward compatibility separately.
\end{enumerate} 
